A Game-Theoretic Framework for Controlled Islanding in the Presence of Adversaries

Controlled islanding effectively mitigates cascading failures by partitioning the power system into a set of disjoint islands. In this paper, we study the controlled islanding problem of a power system under disturbances introduced by a malicious adversary. We formulate the interaction between the grid operator and adversary using a game-theoretic framework. The grid operator first computes a controlled islanding strategy, along with the power generation for the post-islanding system to guarantee stability. The adversary observes the strategies of the grid operator. The adversary then identifies critical substations of the power system to compromise and trips the transmission lines that are connected with compromised substations. For our game formulation, we propose a double oracle algorithm based approach that solves the best response for each player. We show that the best responses for the grid operator and adversary can be formulated as mixed integer linear programs. In addition, the best response of the adversary is equivalent to a submodular maximization problem under a cardinality constraint, which can be approximated up to a $(1-\frac{1}{e})$ optimality bound in polynomial time. We compare the proposed approach with a baseline where the grid operator computes an islanding strategy by minimizing the power flow disruption without considering the possible response from the adversary. We evaluate both approaches using IEEE 9-bus, 14-bus, 30-bus, 39-bus, 57-bus, and 118-bus power system case study data. Our proposed approach achieves better performance than the baseline in about $44\%$ of test cases, and on average it incurs about 12.27 MW less power flow disruption.

==> approx-sol.tex <==
\section{Submodularity Property for Best Response of the Adversary}

In this section, we show that the optimization problem faced by the adversary can be mapped to a submodular maximization problem subject to a cardinality constraint. As a consequence, a greedy algorithm is presented to solve for a pure strategy for the adversary. The greedy algorithm achieves $1-\frac{1}{e}$ optimality guarantee. We relax optimization problem \eqref{eq:adv BR} as follows.
\begin{subequations}\label{eq:adv submodular}
\begin{align}
    \max_{\hat{\mathcal{B}}}~&\sum_{z^o\in\mathcal{Z}^o}\mu(z^o)\left[\sum_{(i,j)\in\hat{\mathcal{L}}}\frac{|P_{i,j}|+|P_{j,i}|}{2}+\sum_{(i,j)\in\tilde{\mathcal{L}}}\frac{|P_{i,j}|+|P_{j,i}|}{2}\right]\label{eq:adv submodular obj}\\
    \text{subject to }~&\hat{\mathcal{L}}=\{(i,j)\in\mathcal{L}:i\in\hat{\mathcal{B}} \text{ or } j\in\hat{\mathcal{B}}\}\label{eq:adv submodular constr 1}\\
    &|\hat{\mathcal{B}}|\leq C\label{eq:adv submodular constr 2}
\end{align}
\end{subequations}
where $\tilde{\mathcal{L}}\subset\mathcal{L}$ is the set of transmission lines tripped by the grid operator when taking action $z^o$. We characterize the relation between optimization problem \eqref{eq:adv expected BR} and \eqref{eq:adv submodular} as follows.
\begin{lemma}\label{lemma:worst case}
Given the strategy of the grid operator, the optimal solution to optimization problem \eqref{eq:adv submodular} is identical to that of optimization problem \eqref{eq:adv expected BR}.
% Given the grid operator's strategies, optimization problem \eqref{eq:adv submodular} computes the worst-case power flow disruption from the adversary's perspective. That is, the optimal value of Eqn. \eqref{eq:adv oracle obj} is a upper bound of that of Eqn. \eqref{eq:adv submodular obj}.
\end{lemma}
\begin{proof}
Using the definition of $z^o$ and $z^a$, objective function \eqref{eq:adv submodular obj} can be rewritten as the same expression of Eqn. \eqref{eq:adv expected BR obj}.

We then prove that constraint \eqref{eq:adv submodular constr 1} represents a subset of feasible solutions of Eqn. \eqref{eq:adv expected BR}. Let $\hat{\mathcal{B}}$ be a feasible solution to optimization problem \eqref{eq:adv submodular}. Let $y$ be defined as $y_i=1$ if $i\in\hat{\mathcal{B}}$ and $y_i=0$ otherwise. Using constraint \eqref{eq:adv submodular constr 1} and the definition of $z^a_{i,j}$, we have that 
\begin{equation*}
    \hat{\mathcal{L}}=\{(i,j)\in\mathcal{L}:i\in\hat{\mathcal{B}}\text{ or } j\in\hat{\mathcal{B}}\}=\{(i,j)\in\mathcal{L}:z_{i,j}^a=0 \text{ if }i\in\hat{\mathcal{B}}\text{ or } j\in\hat{\mathcal{B}}\},
\end{equation*}
which indicates that $y_i+y_j\geq1\implies z_{i,j}^a=0$ for all $i,j\in\mathcal{B}$. We can verify that  $\{(y,z^a):y_i+y_j\geq1\implies z_{i,j}^a=0,~\forall i,j\in\mathcal{B}\}\subseteq\{(y,z^a):z_{i,j}^a+y_i+y_j\geq 1,~\forall i\in\mathcal{B}\}$, and thus constraint \eqref{eq:adv submodular constr 1} represents a subset of Eqn. \eqref{eq:constr adv line indicator 2}.
Combining the arguments above, we have that any feasible solution to Eqn. \eqref{eq:adv submodular} must correspond to a feasible solution of Eqn. \eqref{eq:adv expected BR}.

In the following, we show that $(y,z^a)$ satisfying constraint \eqref{eq:adv submodular constr 1} renders the optimal value of Eqn. \eqref{eq:adv expected BR obj}. We have that given any $z^o$, $(1-z_{i,j}^az_{i,j}^o)=1$ always holds for any feasible solution of Eqn. \eqref{eq:adv submodular} satisfying $y_i+y_j\geq 1$, rendering a positive power flow disruption on transmission line $(i,j)$.
However, $(1-z_{i,j}^az_{i,j}^o)=1$ does not necessarily hold for all feasible solutions of Eqn. \eqref{eq:adv expected BR} since $z_{i,j}^o=z_{i,j}^a=1$ and $y_i+y_j\geq1$ can hold simultaneously without violating Eqn. \eqref{eq:constr adv line indicator 2}, which leads to no power flow disruption on $(i,j)$. Therefore, the optimal solution of Eqn. \eqref{eq:adv submodular} is identical to that of Eqn. \eqref{eq:adv expected BR}.
\end{proof}

In the following, we map optimization problem \eqref{eq:adv submodular} to a problem of maximizing a submodular function subject to a cardinality constraint. We define $\chi_{i,j}(\hat{\mathcal{B}})$ as 
\begin{equation}\label{eq:chi}
    \chi_{i,j}(\hat{\mathcal{B}})=\begin{cases}
    1&\mbox{ if }i\in\hat{\mathcal{B}} \text{ or }j\in\hat{\mathcal{B}}\\
    0&\mbox{ otherwise}
    \end{cases}
\end{equation}
Using the definition of $\chi_{i,j}(\hat{\mathcal{B}})$, optimization problem \eqref{eq:adv submodular} can be rewritten as
\begin{subequations}\label{eq:adv submodular 1}
\begin{align}
    \max_{\hat{\mathcal{B}}}~&\sum_{z^o\in\mathcal{Z}^o}\mu(z^o)\sum_{(i,j)\in\mathcal{L}}\chi_{i,j}(\hat{\mathcal{B}})\frac{|P_{i,j}|+|P_{j,i}|}{2}\label{eq:adv submodular obj 1}\\
    \text{subject to }~&|\hat{\mathcal{B}}|\leq C\label{eq:adv submodular constr 2 1}
\end{align}
\end{subequations}
We have the following result.
\begin{proposition}\label{prop:submodular}
Objective function \eqref{eq:adv submodular obj 1} is submodular and nondecreasing with respect to $\hat{\mathcal{B}}$.
\end{proposition}
\begin{proof}
We first prove Eqn. \eqref{eq:adv submodular obj 1} is submodular with respect to $\hat{\mathcal{B}}$ using the definition of submodularity. Let $\hat{\mathcal{B}}_1\subset\mathcal{B}$ and $\hat{\mathcal{B}}_2\subseteq\hat{\mathcal{B}}_1$. Then using Eqn. \eqref{eq:chi}, we have that
\begin{subequations}
\begin{align}
    \chi_{i,j}(\hat{\mathcal{B}}_1\cup\{h\})-\chi_{i,j}(\hat{\mathcal{B}}_1)=\begin{cases}
    1&\mbox{ if } h=i \text{ or } h=j \text{ and } i,j\notin \hat{\mathcal{B}}_1\\
    0&\mbox{ otherwise}
    \end{cases}\\
    \chi_{i,j}(\hat{\mathcal{B}}_2\cup\{h\})-\chi_{i,j}(\hat{\mathcal{B}}_2)=\begin{cases}
    1&\mbox{ if } h=i \text{ or } h=j \text{ and } i,j\notin \hat{\mathcal{B}}_1\\
    0&\mbox{ otherwise}
    \end{cases}
\end{align}
\end{subequations}
Suppose that $\chi_{i,j}(\hat{\mathcal{B}}_1\cup\{h\})-\chi_{i,j}(\hat{\mathcal{B}}_1)=1$ for $\hat{\mathcal{B}}_1$. Since $\hat{\mathcal{B}}_2\subseteq\hat{\mathcal{B}}_1$, we have that $h=i$ or $h=j$ and $i,j\notin \hat{\mathcal{B}}_2$. Then we have that $\chi_{i,j}(\hat{\mathcal{B}}_2\cup\{h\})-\chi_{i,j}(\hat{\mathcal{B}}_2)=1$. Therefore, we have that
$
    \chi_{i,j}(\hat{\mathcal{B}}_2\cup\{h\})-\chi_{i,j}(\hat{\mathcal{B}}_2)\geq \chi_{i,j}(\hat{\mathcal{B}}_1\cup\{h\})-\chi_{i,j}(\hat{\mathcal{B}}_1)
$ holds for all $\hat{\mathcal{B}}_2\subseteq \hat{\mathcal{B}}_1\subset\hat{\mathcal{B}}$,
which implies that Eqn. \eqref{eq:chi} is submodular with respect to $\hat{\mathcal{B}}$.

Consider $\hat{\mathcal{B}}_2\subset\hat{\mathcal{B}}_1$. Then there must exist some $i\in\hat{\mathcal{B}}_2$ while $i\notin\hat{\mathcal{B}}_2$. Let $j\in\mathcal{B}$ be a substation satisfying $j\notin\hat{\mathcal{B}}_1$. Using Eqn. \eqref{eq:chi}, we have that $\chi_{i,j}(\hat{\mathcal{B}}_2)=0\leq \chi_{i,j}(\hat{\mathcal{B}}_1)=1$. Let $j\in\mathcal{B}$ be a substation satisfying $j\in\hat{\mathcal{B}}_2$. Then we have  that $\chi_{i,j}(\hat{\mathcal{B}}_2)= \chi_{i,j}(\hat{\mathcal{B}}_1)=0$. If $j\in\hat{\mathcal{B}}_1$ holds while $j\notin\hat{\mathcal{B}}_2$ does not hold. Then we have that $\chi_{i,j}(\hat{\mathcal{B}}_2)=0\leq \chi_{i,j}(\hat{\mathcal{B}}_1)=1$. Summarizing the arguments above, we have that Eqn. \eqref{eq:chi} is nondecreasing with respect to $\hat{\mathcal{B}}$.


Combining the arguments above, we have that Eqn. \eqref{eq:adv submodular obj 1} is a summation of non-negative submodular and nondecreasing functions. Therefore, Eqn. \eqref{eq:adv submodular obj 1} is a submodular and nondecreasing function with respect to $\hat{\mathcal{B}}$.
\end{proof}

According to Proposition \ref{prop:submodular}, optimization problem \eqref{eq:adv expected BR} is equivalent to a submodular maximization problem with cardinality constraint. Optimization problem \eqref{eq:adv submodular 1} can be solved efficiently using a greedy algorithm, as shown in Algorithm \ref{algo:greedy}. It has been shown that the greedy algorithm achieves $1-\frac{1}{e}$ optimality guarantee \cite{cornuejols1977exceptional}.
\begin{center}
  	\begin{algorithm}[!htp]
  		\caption{Greedy Algorithm for Eqn. \eqref{eq:adv submodular 1}}
  		\label{algo:greedy}
  		\begin{algorithmic}[1]
  		%	\Procedure{Social\_Max}{$B$}
  			\State $\hat{\mathcal{B}}\leftarrow\emptyset$
  			\While {$|\hat{\mathcal{B}}|\leq C$}
  			\State $i\leftarrow \argmax_{i\in\mathcal{B}\setminus\hat{\mathcal{B}}}\sum_{z^o\in\mathcal{Z}^o}\mu(z^o)\sum_{(i,j)\in\mathcal{L}}[\chi_{i,j}(\hat{\mathcal{B}}\cup\{i\})-\chi_{i,j}(\hat{\mathcal{B}})]\frac{|P_{i,j}|+|P_{j,i}|}{2}$
  			\State $\hat{\mathcal{B}}\leftarrow\hat{\mathcal{B}}\cup\{i\}$
  			\EndWhile
  		%	\EndProcedure
  		\State \Return $\hat{\mathcal{B}}$ and $\{(i,j)\in\mathcal{L}:i\in\hat{\mathcal{B}} \text{ or }j\in\hat{\mathcal{B}}\}$
  		\end{algorithmic}
  	\end{algorithm}
  \end{center}
% The optimality guarantee of Algorithm \ref{algo:greedy} is stated in the following \cite{cornuejols1977exceptional}.
% \begin{lemma}\label{lemma:1-1/e}
% Algorithm \ref{algo:greedy} achieves $(1-\frac{1}{e})$-approximation for optimization problem \eqref{eq:adv submodular 1}.
% \end{lemma}

% We present the optimality of Algorithm \ref{algo:greedy DO} as follows.
% \begin{proposition}
% The grid operator's strategies given by Algorithm \ref{algo:greedy DO} is the minimax strategy.
% \end{proposition}
% \begin{proof}
% By Lemma \ref{lemma:1-1/e}, we have that the adversary plays its $(1-\frac{1}{e})$ best response. As given in \cite{pita2010robust}, the double oracle algorithm gives the minimax strategy for zero-sum game, which is the case in this paper.
% % Assume that Algorithm \ref{algo:greedy DO} terminates at $M+1$-th iteration. Denote the strategies included at line 6 and line 8 of Algorithm \ref{algo:greedy DO} at $M$-th iteration as $(z^{o^M},g^M,\theta^M)$ and $(\hat{\mathcal{B}}^M,\hat{\mathcal{L}}^M)$, respectively. Denote the power flow disruption incurred using strategies $(z^{o},g,\theta)$ and $(\hat{\mathcal{B}},\hat{\mathcal{L}})$ as $H((z^{o},g,\theta),(\hat{\mathcal{B}},\hat{\mathcal{L}}))$. We have that for all $(z^{o},g,\theta)$,
% % \begin{equation*}
% %     H((z^{o},g,\theta),(\hat{\mathcal{B}}^M,\hat{\mathcal{L}}^M))\geq H((z^{o^M},g^M,\theta^M),(\hat{\mathcal{B}}^M,\hat{\mathcal{L}}^M)).
% % \end{equation*}
% % Therefore, we have that
% % \begin{equation*}
% %     \max_{(\hat{\mathcal{B}},\hat{\mathcal{L}})} H((z^{o},g,\theta),(\hat{\mathcal{B}},\hat{\mathcal{L}}))\geq H((z^{o^M},g^M,\theta^M),(\hat{\mathcal{B}}^M,\hat{\mathcal{L}}^M)).
% % \end{equation*}
% % In addition, for all $(\hat{\mathcal{B}},\hat{\mathcal{L}})$, we have that
% % \begin{equation*}
% %   (1-\frac{1}{e})\max_{(\hat{\mathcal{B}},\hat{\mathcal{L}})} H((z^{o^M},g^M,\theta^M),(\hat{\mathcal{B}},\hat{\mathcal{L}}))\leq H((z^{o^M},g^M,\theta^M),(\hat{\mathcal{B}}^M,\hat{\mathcal{L}}^M)).
% % \end{equation*}
% % Thus, the following relation holds for all $(z^{o},g,\theta)$:
% % \begin{equation*}
% %     (1-\frac{1}{e})\max_{(\hat{\mathcal{B}},\hat{\mathcal{L}})} H((z^{o^M},g^M,\theta^M),(\hat{\mathcal{B}},\hat{\mathcal{L}}))\leq\max_{(\hat{\mathcal{B}},\hat{\mathcal{L}})} H((z^{o},g,\theta),(\hat{\mathcal{B}},\hat{\mathcal{L}}))
% % \end{equation*}
% % Therefore, 
% \end{proof}


